Peripheral Vision Transformer

Human vision possesses a special type of visual processing systems called peripheral vision. Partitioning the entire visual field into multiple contour regions based on the distance to the center of our gaze, the peripheral vision provides us the ability to perceive various visual features at different regions. In this work, we take a biologically inspired approach and explore to model peripheral vision in deep neural networks for visual recognition. We propose to incorporate peripheral position encoding to the multi-head self-attention layers to let the network learn to partition the visual field into diverse peripheral regions given training data. We evaluate the proposed network, dubbed PerViT, on ImageNet-1K and systematically investigate the inner workings of the model for machine perception, showing that the network learns to perceive visual data similarly to the way that human vision does. The performance improvements in image classification over the baselines across different model sizes demonstrate the efficacy of the proposed method.

==> mustreflist.tex <==


\jmin{Transformer-based models:}
\begin{itemize}
    \item ViT: \cite{dosovitskiy2021vit}
    \item DeiT: \cite{touvron2021deit}
    \item ConViT: \cite{d2021convit}
    \item Swin:\cite{liu2021swin}
    \item CvT: \cite{wu2021cvt}
    \item PVT: \cite{wang2021pvt}
    \item SASA: \cite{ramachandran2019sasa}
    \item HaloNet: \cite{vaswani2021halonet}
    \item AttentionIsAllYouNeed: \cite{vaswani2018attention}
    \item BERT: \cite{devlin2019bert}
    \item DETR: \cite{carion2020detr}
    \item Segmenter: \cite{strudel2021segmenter}
    \item OnTheRelationship: \cite{cordonnier2021ontherelationship}
    \item Perceiver: \cite{jaegle2021perceiver}
    \item Performer: \cite{choromanski2021performer}
    \item DINO: \cite{caron2021dino}
    \item CPVT: \cite{chu2021cpvt}
    \item BoTNet: \cite{srinivas2021botnet}
    \item GPT 1-3:
    \item Infty-former: 
    \item Searching for TrioNet: Combining Convolution with Local and Global Self-Attention
    \item A ConvNet for the 2020s
    \item CoAtNet: Marrying Convolution and Attention for All Data Sizes
    \item Augmenting Convolutional Networks with Attention-based Aggregation
    \item 
    \item 
\end{itemize}

\smallbreak\noindent\textbf{Position encoding.} 

\begin{itemize}
    \item Shaw's RPE: \cite{shaw2018selfattention}
    \item transformer-XL: \cite{dai2019transformerXL}
    \item iRPE: \cite{wu2021irpe}
    \item Huang's RPE: \cite{huang2020rpe}
    \item RPE in SASA: \cite{ramachandran2019sasa}
    \item Axial-Deeplab: \cite{wang2020axialdeeplab}
    \item 
    \item Relative Positional Encoding for Transformers with Linear Complexity (ICML 2021)
    
    
\end{itemize}


\smallbreak\noindent\textbf{Peripheral vision.} 



\jmin{Peripheral vision in computer vison literature.:}
\begin{itemize}
    \item Biological Plausibility \cite{harrington2022bio}
    \item Neurocomputational modeling \cite{wang2017central}
    \item Obj rec \& tracking \cite{gould2007peripheral}
    \item Biologically inspired \cite{lukanov2021bio}
    \item Recognition test \cite{chin2012object}
    \item
\end{itemize}

\jmin{Misc.:}
\begin{itemize}
    \item EfficientNet: \cite{tan2019efficientnet}
    \item earlyConvSeeBetter: \cite{xiao2021early}
    \item ViTseeLikeCNN?: \cite{raghu2021dovitseecnn}
    \item NotAllViT: \cite{wang2021notall16x16}
    \item 
\end{itemize}
